On the Power of Delayed Flexibility: Balls, Bins, and a Few Opaque Promotions

Effective load balancing lies at the heart of many applications in operations. Frequently tackled via the balls-into-bins paradigm, seminal results established the power of two choices in load balancing: a limited amount of costly flexibility goes a long way in order to maintain an approximately balanced load throughout the decision-making horizon. In many applications, however, balance across time may be too stringent a requirement; rather, the only desideratum is approximate balance at the {\it end} of the horizon. Motivated by this observation, in this work we design "delayed-flexibility" algorithms tailored to such settings. For the canonical balls-into-bins problem, we show that a simple policy that begins exerting flexibility toward the end of the time horizon - namely, when $\Theta\left(\sqrt{T\log T}\right)$ periods remain - suffices to achieve an approximately balanced load, i.e., a maximum load within $O(1)$ of the average load. Moreover, with just a small amount of adaptivity, a threshold policy achieves the same result, while only exerting flexibility in $O\left(\sqrt{T}\right)$ periods, thus matching a natural lower bound. We leverage these results to study the design of opaque selling strategies in retail settings, a topic recently identified as a key application of the power of two choices paradigm. For this problem, we prove that late-stage opaque selling strategies achieve the optimal trade-off between exerting costly flexibility - i.e., offering the opaque product at a discount - and achieving inventory cost savings through load balancing. We demonstrate the robustness of our insights via extensive numerical experiments, for a variety of customer choice models.

==> static-opaque-selling.tex <==
\subsection{Analysis of the Static Opaque Selling Policy}\label{apx:opaque-static}

\chcomment{come back this}

In this section, our goal is to show that the expected length of a replenishment cycle under the static opaque selling policy $\pis$ is within an additive constant of the maximum possible cycle length $N(S-1)+1$. This is formalized in the following theorem.
\begin{theorem} \label{thm:opaque-static}
The static opaque selling policy $\pis$ with $\cststatic = \frac{2\sqrt{6}N(N-1)(N+1)}{q_o}+4N$ and $\delta \in \Theta(1)$ ensures $\mathbb{E}[\Rs] = NS - \thetas, \text{where } \thetas \in \mathcal{O}(1).$
\end{theorem}

We state the auxiliary results in Appendix \ref{app:preparation} and defer the proof of \cref{thm:opaque-static} to Appendix \ref{app:static}. As in the analysis of the semi-dynamic policy, in this proof we assume that, if the customer purchases the opaque product, the retailer sellers 2 out of the $N$ products uniformly at random, and allocates the product with the higher remaining inventory.





\subsubsection{Proof of \texorpdfstring{\cref{thm:opaque-static}}{Lg}} \label{app:static}
\begin{proof}{Proof of \cref{thm:opaque-static}.}
Notice that the assumptions $\delta \in \Theta(1)$ and $\delta > \parenthesis{\frac{1}{4} - \frac{1}{2N}}\cdot \gamma$ imply that $q_o \in (0,1]$ is independent of $S$. We use $q := q_o$ for notational simplicity throughout this proof.

Applying \cref{prop:final_relation} to the static policy, we obtain $$\mathbb{E}[\Rs] = N(S-1)+2 - \sum_{t = S}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N).$$ Thus, to prove \cref{thm:opaque-static}, it suffices to show that
\begin{equation}\label{eq:static_main}
    \sum_{t = S}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N) \in \mathcal{O}(1).
\end{equation}

Recall $\cststatic = \frac{2\sqrt{6}N(N-1)(N+1)}{q}+4N, \staticcst = \frac{2\sqrt{6}N(N-1)}{q},$ and $\That = T - \cststatic \cdot \sqrt{T \log(T)}.$
Moreover, as illustrated in \cref{fig:illu1}, we decompose $\cststatic$ into $\cststatica$ and $\staticcst$, where $\cststatica = \cststatic-\staticcst= \frac{2\sqrt{6}N(N-1)N}{q}+4N$. Let $\Ttilde := T - \cststatica \cdot \sqrt{T \log(T)},$ so that $T - \Ttilde = \cststatica \sqrt{T\log(T)}$ and $\Ttilde - \That = \staticcst \sqrt{T\log(T)}.$

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{Plots/illustration 1.png}
    \caption{\centering Illustration of $\That, \Ttilde$ and $T$}
    \label{fig:illu1}
\end{figure}


By construction, opaque selling starts at $\That$. We leverage the definition of $\Ttilde$ to prove \eqref{eq:static_main} by considering $t \leq \Ttilde$ and $t > \Ttilde$ separately. For $t \leq \Ttilde$,
\begin{align*}
    \mathbb{P}(\Gaps(t) \geq S-t/N) = \mathbb{P}(\max_j \xstatic_j(t) \geq S) \leq \mathbb{P}(\max_j \xstatic_j(\Ttilde) \geq S).
\end{align*}

We make the following claim and defer its proof to Appendix \ref{app:auxi}.

\begin{claim1}\label{cl:static_prob}
$\mathbb{P}(\max_j \xstatic_j(\Ttilde) \geq S) \leq \frac{a_1}{T^2}$ for some constant $a_1 > 0.$
\end{claim1}

Then, we have:
\begin{align*}
    \sum_{t = S}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N) &= \sum_{t = S}^{\Ttilde} \mathbb{P}(\Gaps(t) \geq S- t/N) + \sum_{t = \Ttilde+1}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N)\\
    &\leq T\cdot \frac{a_1}{T^2} +  \sum_{t = \Ttilde+1}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N)\\
    &= \frac{a_1}{T} + \sum_{t = \Ttilde+1}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N).
\end{align*}

Thus, it suffices to show that 
\begin{equation} \label{eq:repeated_part}
    \sum_{t = \Ttilde+1}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N) \leq a_2,
\end{equation}
for some constant $a_2 > 0$.


Now, as in the balls-into-bins model, for $i,j \in [N]$, we define
\begin{align*}
E_{ij}^1 := &\left\{\history{\Ttilde} \in \historyset{\Ttilde}\mid i \in \arg\max_{k\in[N]} \xstatic_k(\Ttilde), j \in \arg\min_{k\in[N]} \xstatic_k(\Ttilde), \xstatic_i(t) \neq \xstatic_j(t), \forall \ t \in \{\That,...,\Ttilde\}\right\} \\
E_{ij}^2 := &\{\history{\Ttilde} \in \historyset{\Ttilde}\mid i \in \arg\max_{k\in[N]} \xstatic_k(\Ttilde), j \in \arg\min_{k\in[N]} \xstatic_k(\Ttilde), \\
&\hspace{2.7cm}\xstatic_i(t) = \xstatic_j(t) \text{ for some } t \in \{\That,...,\Ttilde-1\},\xstatic_i(\Ttilde) \neq \xstatic_j(\Ttilde)\}
\end{align*}

It follows %is easy to check 
that $E_{ij}^1$ and $E_{ij}^2$ satisfy the conditions for $F_{ij}^1$ and $F_{ij}^2$ in \cref{lem:inventory_bound} with $t_1 = \That$ and $t_2 = \Ttilde$. Thus, applying \cref{lem:inventory_bound}, we obtain
\begin{align}\label{eq:inventory_main}
    \sum_{t = \Ttilde+1}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N) &=  \sum_{t = \Ttilde+1}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N \mid \That, \Ttilde) \\
    &\leq a_3 + \sum_{t = \Ttilde+1}^{N(S-1)+1}\sum_{i,j}\mathbb{P}(E_{ij}^1 \mid \That, \Ttilde) = a_3 + \sum_{t = \Ttilde+1}^{N(S-1)+1}\sum_{i,j}\mathbb{P}(E_{ij}^1)
\end{align}
for some constant $a_3 > 0$. Notice that both the first and the second equality above hold because $\That$ and $\Ttilde$ are deterministic quantities that provide no additional information on the gap.

To bound $\mathbb{P}(E_{ij}^1)$, since %\chcomment{I think no need to define $\staticcst$, just immediately use $\staticcst$} \kzcomment{addressed.}
$\Ttilde - \That = \staticcst \sqrt{T\log(T)} \geq \staticcst \sqrt{\Ttilde\log(\Ttilde)},$
%it is easy to check 
we observe that $E_{ij}^1$ satisfies the condition for $F_{ij}^1$ in \cref{lem:e1ij} with $t_1 = \That$ and $t_2 = \Ttilde.$ Thus, applying \cref{lem:e1ij}, we obtain $$\PP{E_{ij}^1} \leq \beta \That^{-2} + e^{-\alpha_1 (\Ttilde - \That)}.$$ Plugging this result back into \eqref{eq:inventory_main}, we obtain
\begin{align*}
    \sum_{t = \Ttilde+1}^{N(S-1)+1} \mathbb{P}(\Gaps(t) \geq S- t/N) &\leq a_3 + \sum_{t = \Ttilde+1}^{N(S-1)+1}\sum_{i,j}(\beta T^{-2} + e^{-\alpha_1 (\Ttilde - \That)})\\
    &\leq a_3 +T \sum_{i,j}(\beta T^{-2} + e^{-\alpha_1 (\Ttilde - \That)}) \leq a_2
\end{align*}
for some constant $a_2$ and large enough $T,$ where the second inequality comes from the fact that $$N(S-1)+1 - \Ttilde \leq N(S-1)+1 = T.$$ %This completes the proof.
\end{proof}

% \subsubsection{Proof of \texorpdfstring{\cref{cor:opaque-static}}{Lg}}

% \begin{proof}{Proof.}
% From \cref{prop:ordering} (iii), \cref{prop:holding} (iii) and \cref{prop:discount}~(iii), we have
% \begin{align*}
%     \Cs &= \Ks +\Hs +\Ds
%     \leq \frac{K}{NS-\thetas} + \frac{h}{2}\left(NS+1 + \thetas\right) + \delta q \cdot \thetaf,
% \end{align*}
% where $\thetas \in \mathcal{O}(1), \thetaf \in \Theta\left(\sqrt{\frac{\log S}{S}}\right)$.
% % \hfill\qed
% \end{proof}

\subsubsection{Proofs of Auxiliary Results} \label{app:auxi}


\begin{proof}{Proof of Claim \ref{cl:static_prob}.}
To prove the claim, we first show that 
\begin{align}\label{eq:static_prob1}
    \mathbb{P}(\max_j \xstatic_j(\Ttilde) \geq S) \leq \mathbb{P}(\max_j \xnf_j(\Ttilde) \geq S - \staticcst \sqrt{T \log(T)}).
\end{align}
%\chcomment{What's $x_j(\Ttilde)$? No-flex?} \kzcomment{addressed.}


{
For \eqref{eq:static_prob1}, note that $\max_j \xstatic_j(\Ttilde) \geq S$ implies $\max_j \xstatic_j(\That) \geq S - \staticcst \sqrt{T \log(T)}$, since in the worst case all balls from $\That$ to $\Ttilde$ go into $\argmax_j \xstatic_j(\That)$. Thus, $$\mathbb{P}(\max_j \xstatic_j(\Ttilde) \geq S) \leq \mathbb{P}(\max_j \xstatic_j(\That) \geq S - \staticcst \sqrt{T \log(T)}).$$}
Since the no-flex policy and the static policy are the same before $\That,$ we also have:
\begin{align*}
    \mathbb{P}(\max_j \xstatic_j(\That) \geq S - \staticcst \sqrt{T \log(T)})
    &= \mathbb{P}(\max_j \xnf_j(\That) \geq S - \staticcst \sqrt{T \log(T)})\\
    &\leq \mathbb{P}(\max_j \xnf_j(\Ttilde) \geq S - \staticcst \sqrt{T \log(T)}),
\end{align*}
{where the inequality follows from the fact that $\Ttilde \geq \That \implies \max_j \xnf_j(\Ttilde) \geq \max_j \xnf_j(\That)$.}
% \chdelete{where the inequality comes from the monotonicity of $x_j(t)$ with respect to $t$ on every sample path. We are thus done with \eqref{eq:static_prob1}.}

We now argue that
\begin{align}\label{eq:static_prob2}
    \mathbb{P}(\max_j \xnf_j(\Ttilde) \geq S - \staticcst \sqrt{T \log(T)}) \leq \frac{a_1}{T^2}
\end{align}
for some constant $a_1 > 0$ to conclude the proof of the claim.

Recall, $\cststatica = \frac{2\sqrt{6}N(N-1)N}{q}+4N$ and $\staticcst = \frac{2\sqrt{6}N(N-1)}{q}$, so $\cststatica = N(\staticcst+4).$ For large enough $T,$ %We have
\begin{align}
    \mathbb{P}(\max_j \xnf_j(\Ttilde) \geq S - \staticcst \sqrt{T \log(T)})
    &\leq N \mathbb{P}\left(B(T - \cststatica \sqrt{T \log(T)},\frac{1}{N}) \geq \frac{T-N \cdot \staticcst \sqrt{T \log(T)}}{N}\right) \notag \\
    &= N \mathbb{P}\left(B(T - \cststatica \sqrt{T \log(T)},\frac{1}{N}) \geq (1+\epsilon) \frac{T-\cststatica \sqrt{T \log(T)}}{N}\right), \label{eq:claim1-chernoff}
\end{align}
where $$\epsilon = \frac{(\cststatica-N\staticcst) \sqrt{T \log(T)}}{T - \cststatica \sqrt{T \log(T)}} = \frac{4N\sqrt{T\log T}}{T-c_{static}^1\sqrt{T\log T}}.$$ 
The first inequality above follows from $SN > T = N(S-1)+1,$ which yields $$S - \staticcst \sqrt{T \log(T)} = \frac{NS-N \cdot \staticcst \sqrt{T \log(T)}}{N} \geq \frac{T-N \cdot \staticcst \sqrt{T \log(T)}}{N}.$$ Then, applying the Chernoff bound to \eqref{eq:claim1-chernoff} we obtain:
\begin{align*}
    \mathbb{P}(\max_j \xnf_j(\Ttilde) \geq S - \staticcst \sqrt{T \log(T)})
    &\leq \exp\left(-\frac{\epsilon^2}{2+\epsilon} \frac{T-\cststatica \sqrt{T \log(T)}}{N}\right)\\
    &= \exp\left(-\frac{(\cststatica - N \staticcst)^2 T \log(T)}{2N (T - \cststatica \sqrt{T \log(T)}) + N (\cststatica - N \staticcst)\sqrt{T \log(T)}}\right)\\
    &\leq \exp\left(-\frac{16 N^2 T \log(T)}{2NT + 4N^2 \sqrt{T \log(T)}}\right)\\
    &\leq e^{-\frac{16 \log(T)}{6}} \leq \frac{a_1}{T^2}
\end{align*}
for some constant $a_1 > 0.$ For the second inequality above we plug in values of $\cststatica$, $\staticcst$, and upper bound $(T - \cststatica \sqrt{T \log(T)})$ by $T.$
\end{proof}


